Performance Analysis of IEEE 802.11p Preamble Insertion in C-V2X Sidelink Signals for Co-Channel Coexistence

Spectrum scarcity is one of the main challenges of future wireless technologies. When looking at vehicle-to-everything (V2X), this is amplified as spectrum sharing could impact road safety and traffic efficiency. It is therefore of particular importance to study solutions that allow the coexistence, in the same geographical area and in the same channels, of what are today the main V2X access technologies, namely IEEE 802.11p and sidelink LTE-V2X Mode 4. In this work, in addition to investigating the impact of the reciprocal interference, which we demonstrate to have a strong impact especially on the first and in congested channel conditions, a mitigation solution is extensively studied, which is based on the insertion of the IEEE 802.11p preamble at the beginning of the LTE-V2X sidelink transmission. The proposal, which is also under discussion within the standardization bodies, requires no modifications to the IEEE 802.11p protocol stack and minor changes to LTE-V2X sidelink. This solution is directly applicable to upcoming IEEE 802.11bd and extendable to NR-V2X sidelink. The paper shows, through analysis and simulations in free-flow and dense scenarios, that the proposal allows for a mitigation of collisions caused by co-channel coexistence under low to high-load channel conditions and that the improvement is also granted in congested cases when combined with additional countermeasures. Regarding the latter aspect, in particular, different approaches are compared, demonstrating that acting on the congestion control mechanisms is a simple but effective solution.

==> TableMetrics.tex <==
\begin{table}%[!t]
\caption{Output metrics.
\vspace{-2mm}
\label{Tab:metrics}}
\footnotesize
%\scriptsize
\centering
\begin{tabular}{p{1cm}p{6cm}}
\hline \hline
Packet reception ratio (PRR) & Average ratio between the number of vehicles at a certain distance from the transmitter that are correctly decoding a packet and the overall number of vehicles at the same distance; PRR is calculated with a granularity of 10~m.\\
Data age (DA) & corresponding to the time elapsed from the generation of a correctly received packet and the next correctly decoded one by the same receiver; it implicitly accounts for the allocation delay and the correlation among errors; DA is evaluated for all transmissions within 400~m.\\
\hline \hline
\end{tabular}
%\vskip -0.4cm
\end{table}


==> TableSettingsTWC.tex <==
%\begin{table}%[!t]
\begin{table}%[!t]
\caption{Main adopted parameters and settings.
\vspace{-2mm}
\label{Tab:Settings}}
%\footnotesize
\scriptsize
\centering
%\begin{tabular}{p{3.3cm}p{4.7cm}}
%\begin{tabular}{p{5cm}p{7cm}}
\begin{tabular}{p{3cm}p{4.6cm}}
\hline \hline
%\textbf{Common parameters (Symbol)} & \textbf{Value} \\  
%\hline
%\textbf{\textit{Scenario}} & \\
%Simulated time ($\Tsim$) & 90 s \\
%Position of vehicles & Highway \\
\textbf{\textit{Common settings}} & \\
Scenario & 3+3 lanes highway, 2~km straight road\\
Density & Variable \\
Speed & 70 km/h \\
Beacon periodicity & Following CAM rules \cite{3GPP_EN_302_637_2} \\
Beacon size & 350~B \\
Channels & ITS bands at 5.9 GHz \\
Bandwidth & 10 MHz \\
Transmission power & 23~dBm \\
Antenna gain (tx and rx)  & 3 dB \\
Noise figure & 6~dB \\
Propagation model & WINNER+, Scenario B1 \\
Shadowing & Variance 3 dB, decorr. dist. 25~m \\ \hline
\textbf{\textit{IEEE~802.11p}} & \\
MCS & 2 (QPSK, 1/2), PER=0.1@SINR=3.1dB \\
Duration of the initial space & 110\;$\mu$s \cite{ETSI_TS_102_636} \\
Random backoff & $[0\div 15] \cdot 13$\;$\mu$s \cite{ETSI_TS_102_636} \\ 
Carrier sensing threshold & -65 dBm \\
Preamble detection threshold & -100 dBm \\
Congestion control & ETSI DCC \cite{ETSI_EN_302_663} \\
\hline
\textbf{\textit{Sidelink LTE-V2X Mode 4}} & \\
%MCS & \hbox{11 (16-QAM, 0.41),} PER=0.1@SINR=7.4dB \\
MCS & 11 (16-QAM, 0.41), PER=0.1@SINR=7.4dB \\
Subchannel size & 10 resource block pairs \cite{ETSI_TS_103_613} \\
Number of subchannels & 5 \\
Subchannels per packet & 2 \\
Configuration & Adjacent \\
Keep probability & 0.5 \\
Allocation periodicity & 100 ms \\
Suchannel sensing threshold & -110~dBm \\
Congestion control & ETSI CC for LTE-V2X \cite{ETSI_103_574} \\
HARQ & Blind retransmission if CC allows \\
\hline \hline
\end{tabular}
%\vskip -0.4cm
\end{table}


==> TableSymbols.tex <==
\begin{table}%[!t]
\caption{Main symbols. 11p for IEEE 802.11p, LTE for LTE-V2X.
\vspace{-2mm}
\label{Tab:symbols}}
\footnotesize
%\scriptsize
\centering
\begin{tabular}{p{0.6cm}p{7cm}}
\hline \hline
%\textbf{Common parameters (Symbol)} & \textbf{Value} \\  
%\hline
%\textbf{\textit{Scenario}} & \\
%Simulated time ($\Tsim$) & 90 s \\
%Position of vehicles & Highway \\
%\textbf{\textit{Common settings}} & \\
$\PRR$ & Packet error rate\\
$\PRRbusy$ & Packet error rate given that the current TTI is sensed busy\\
$\PRRcurrent$ & Packet error rate given that the current TTI is sensed idle and the transmission ends in current TTI\\
$\PRRsubseq$ & Packet error rate given that the current TTI is sensed idle and the transmission ends in subsequent TTI\\
$\PRRunprotected$ & Packet error rate given that the sensing procedure is not used\\
$\Ppos(x)$ & Prob. that the main LTE interferer is in the position $x$ \\
$\Pwithin$ & Prob. that the 11p transmission ends in current TTI \\ 
$\Pcross$ & Prob. that the 11p transmission ends in subsequent TTI \\
$\Psensed$ & Prob. that the current TTI is sensed busy by 11p\\
$\Pnotswithin$ & Prob. that the 11p transmission ends in current TTI and the current TTI is sensed idle \\ 
$\Pnotscross$ & Prob. that the 11p transmission ends in subsequent TTI and the current TTI is sensed idle \\ 
\hline \hline
\end{tabular}
%\vskip -0.4cm
\end{table}

